Speculative Action Generation for World Action Models

World Action Models (WAMs) have shown strong capabilities in robotic manipulation by jointly predicting actions and future visual observations. However, iterative denoising incurs high inference latency, hindering continuous robot control in real time. Although recent methods have reduced the cost of visual prediction at inference, action denoising still requires multiple sequential calls to the action diffusion transformer (DiT) and accounts for over 70% of total inference latency. To address this bottleneck, we propose Speculative Action Generation (SAG), a plug-and-play speculative sampling framework that enables multiple denoising steps per action DiT call without additional training or auxiliary models. Specifically, SAG implements two alternative algorithms: (1) SAG-Residual adapts speculative sampling to deterministic action denoising using a local residual criterion for acceptance and Euler updates for correction. (2) SAG-Coupling reformulates action denoising as a stochastic differential equation to enable probabilistic acceptance and uses coupling for correction. Extensive experiments on simulated and real-world tasks demonstrate that SAG accelerates WAM action generation by $1.7$--$3.3\times$ with comparable task performance and can be extended to flow-based vision language action (VLA) models with up to a $2.9\times$ speedup on $\pi_{0.5}$. Our project page is available at https://sag-wam.github.io/.

==> title_layout.tex <==
\makeatletter
\let\sag@original@maketitle\@maketitle
\let\sag@compact@maketitle\@maketitle
\newdimen\sag@titleoffset
\patchcmd{\sag@compact@maketitle}{\vskip .375in}{\vskip\sag@titleoffset\kern0pt}{}{\PackageError{sag}{Title top spacing patch failed}{}}
\patchcmd{\sag@compact@maketitle}{\Large \bf \@title}{\fontsize{16}{19.2}\selectfont\bfseries\@title}{}{\PackageError{sag}{Title font patch failed}{}}
\patchcmd{\sag@compact@maketitle}{\vspace*{24pt}}{\vspace*{16pt}}{}{\PackageError{sag}{Title author spacing patch failed}{}}
\patchcmd{\sag@compact@maketitle}{\vskip .5em}{\vskip 0pt}{}{\PackageError{sag}{Author bottom spacing patch failed}{}}
\patchcmd{\sag@compact@maketitle}{\vspace*{12pt}}{\vspace*{6pt}}{}{\PackageError{sag}{Title bottom spacing patch failed}{}}
\newdimen\sag@titlepadding
\def\@maketitle{%
  \begingroup
    \sag@titleoffset=0pt
    \setbox0=\vbox{\hsize\textwidth
      \def\@author{Anonymous CVPR submission}%
      \sag@original@maketitle}%
    \sag@titlepadding=\dimexpr\ht0+\dp0\relax
    \typeout{SAG original title height: \the\sag@titlepadding}%
    \setbox0=\vbox{\hsize\textwidth\sag@compact@maketitle}%
    \typeout{SAG compact title height: \the\dimexpr\ht0+\dp0\relax}%
    \advance\sag@titlepadding by -\dimexpr\ht0+\dp0\relax
    \ifdim\sag@titlepadding<0pt
      \sag@titleoffset=\sag@titlepadding
      \sag@titlepadding=0pt
    \fi
    \ifdim\sag@titleoffset<-46pt
      \PackageError{sag}{Author block exceeds the available upper-page space}{Reduce only title-area spacing.}%
    \fi
    \typeout{SAG title offset: \the\sag@titleoffset}%
    \typeout{SAG title padding: \the\sag@titlepadding}%
    \sag@compact@maketitle
    \vskip\sag@titlepadding
  \endgroup
}
\makeatother

